PTSan: A Practical Memory Safety Sanitizer for C/C++ with Pointer-Object Authority

Memory safety errors remain the dominant source of severe vulnerabilities in C and C++. Pointer-based sanitizers provide stronger guarantees than location-based tools such as LLVM's ASan, but their overhead and compatibility limitations have constrained production use. We present PTSan, an LLVM sanitizer that makes pointer-based checking practical by storing an object identifier in each pointer's high bits and its bounds in a fixed-size runtime table. This representation trades a finite live-object budget for low overhead, optimizer visibility, and commodity-hardware support. Because identity travels with the pointer value, ordinary LLVM dataflow propagates it without explicit per-pointer metadata instructions. Separating metadata lookup from check enforcement exposes both as LLVM IR, enabling check hoisting, elision, and merging, plus whole-function min-cut placement of compatibility tag strips. Intel Linear Address Masking eliminates the remaining strips in hardware when available. On stock hardware PTSan runs at parity with the fastest published location-based sanitizer: 57.2% geomean overhead on SPEC CPU 2017 on x86-64 (46.4% with Intel LAM), 54.7% on ARM64, and 31.5% (x86-64) on the application-shaped LLVM MultiSource suite. This is roughly a third of the published overhead percentage of prior systems with similar pointer-object authority guarantees, while preserving the inter-object, non-object, and temporal detection coverage measured by an independent memory safety test suite. Its physical-memory overhead is effectively native, a critical property for production deployment as memory costs become a first-order constraint. We also demonstrate practical overhead on real-world server and security workloads. These results show that PTSan brings practical pointer-based memory safety into a recompile-only sanitizer deployment model.

==> eval/generated/tab-llvm-full-body.tex <==
\begin{tabular}{@{}lrrrr@{\hskip 6pt}@{}lrrrr@{\hskip 6pt}@{}lrrrr@{}}
  \toprule
  Program & x86 & LAM & ARM & IDs & Program & x86 & LAM & ARM & IDs & Program & x86 & LAM & ARM & IDs \\
  \midrule
  alacconvert-decode & 2.2\% & 14.6\% & -20.0\% & 7 & qbsort & 147.5\% & 141.2\% & 137.1\% & 2 & ControlLoops-flt & -1.0\% & -0.4\% & 3.3\% & 11 \\
  alacconvert-encode & 6.7\% & 2.1\% & 0.0\% & 10 & testtrie & -- & -- & -- & 5,359 & CrossingThresholds-dbl & -3.1\% & -1.9\% & 6.1\% & 11 \\
  clamscan & 43.1\% & 34.5\% & 51.2\% & 63k & bisect & 2.8\% & 1.3\% & 3.0\% & 5 & CrossingThresholds-flt & 0.6\% & 3.1\% & 8.4\% & 11 \\
  ldecod & 65.6\% & 54.4\% & 128.6\% & 4,257 & eks & -- & -- & -- & 108 & Equivalencing-dbl & 1.1\% & -0.1\% & -2.1\% & 11 \\
  lencod & 65.4\% & 54.8\% & 131.7\% & 9,069 & main & 9.3\% & 8.9\% & 87.5\% & 2 & Equivalencing-flt & 1.6\% & 1.8\% & 0.6\% & 11 \\
  SIBsim4 & 55.1\% & 45.8\% & 93.8\% & 641k & vor & 37.0\% & 30.9\% & 72.9\% & 200k & Expansion-dbl & 2.2\% & 0.9\% & 1.8\% & 11 \\
  SPASS & 45.9\% & 29.1\% & 78.2\% & 2 & iotest & -6.0\% & 5.6\% & 111.5\% & 1 & Expansion-flt & -0.0\% & 0.4\% & 1.1\% & 11 \\
  aha & 77.2\% & 45.8\% & 97.3\% & 8 & bintr & 32.3\% & 21.2\% & 54.8\% & 46k & GlobalDataFlow-dbl & 0.9\% & 0.9\% & -0.7\% & 11 \\
  make\_dparser & 157.4\% & 140.4\% & 142.9\% & 2 & imp & 82.1\% & 77.8\% & 74.1\% & 1,548 & GlobalDataFlow-flt & 2.1\% & -0.9\% & -1.1\% & 11 \\
  hbd & -- & -- & -- & 7,812 & automotive-basicmath & 137.9\% & 135.8\% & 81.3\% & 2 & IndirectAddressing-dbl & 0.8\% & 1.5\% & 6.0\% & 11 \\
  hexxagon & 49.8\% & 49.2\% & 83.8\% & 137 & automotive-bitcount & 4.6\% & 0.0\% & 2.9\% & 0 & IndirectAddressing-flt & 2.0\% & 0.1\% & 11.9\% & 11 \\
  kc & 176.9\% & 183.8\% & 142.9\% & 2 & automotive-susan & 80.5\% & 86.7\% & 83.3\% & 2 & InductionVariable-dbl & 0.6\% & 0.1\% & 6.9\% & 11 \\
  lambda & 128.2\% & 97.4\% & 534.0\% & 3,195 & consumer-jpeg & -- & -- & -- & 14 & InductionVariable-flt & 1.5\% & -0.0\% & 10.1\% & 11 \\
  lua & 123.9\% & 91.3\% & 173.1\% & 2 & consumer-lame & 62.3\% & 60.3\% & 34.1\% & 305 & LinearDependence-dbl & 0.3\% & -0.9\% & -1.4\% & 11 \\
  minisat & 71.0\% & 57.7\% & 98.0\% & 380k & consumer-typeset & 144.9\% & 109.6\% & 160.5\% & 2,826 & LinearDependence-flt & 1.2\% & 2.3\% & -0.6\% & 11 \\
  Obsequi & 28.5\% & 24.2\% & 31.1\% & 154 & network-dijkstra & 54.0\% & 28.9\% & 68.0\% & 331 & LoopRerolling-dbl & 0.1\% & 0.1\% & 2.9\% & 11 \\
  oggenc & 37.8\% & 32.0\% & 50.0\% & 3,990 & network-patricia & 98.2\% & 103.6\% & 80.8\% & 2 & LoopRerolling-flt & 0.6\% & 0.7\% & 2.4\% & 11 \\
  sgefa & 4.9\% & 2.5\% & 12.5\% & 611 & security-rijndael & 16.0\% & 18.9\% & 11.1\% & 2 & LoopRestructuring-dbl & -0.8\% & -1.0\% & 0.0\% & 11 \\
  siod & -- & -- & -- & 174 & security-sha & 0.0\% & -7.3\% & -- & 1 & LoopRestructuring-flt & -6.2\% & -1.6\% & -0.0\% & 11 \\
  spiff & 51.4\% & 48.6\% & 70.4\% & 22.3M & telecomm-CRC32 & 55.4\% & 47.5\% & 46.5\% & 0 & NodeSplitting-dbl & -0.0\% & -0.0\% & 0.4\% & 11 \\
  sqlite3 & 142.9\% & 118.6\% & 252.6\% & 18k & telecomm-fft & 103.6\% & 97.6\% & 70.0\% & 2 & NodeSplitting-flt & -0.5\% & -0.3\% & -0.1\% & 11 \\
  viterbi & 59.6\% & 53.3\% & 64.2\% & 9 & telecomm-gsm & 15.8\% & 7.7\% & 14.6\% & 2 & Packing-dbl & 27.8\% & 27.2\% & 19.0\% & 11 \\
  7zip-benchmark & 24.6\% & 20.4\% & 38.8\% & 285 & is & 0.2\% & 0.3\% & 5.1\% & 20 & Packing-flt & 31.8\% & 30.6\% & 32.3\% & 11 \\
  smg2000 & 39.8\% & 36.8\% & 27.9\% & 89k & bh & 13.5\% & 13.4\% & 36.1\% & 29k & Recurrences-dbl & 0.1\% & -0.0\% & 1.4\% & 11 \\
  AMGmk & 47.8\% & 42.6\% & 65.6\% & 12 & bisort & 21.0\% & 17.1\% & 49.1\% & 524k & Recurrences-flt & 0.1\% & 0.0\% & 0.1\% & 11 \\
  CrystalMk & 70.1\% & 73.7\% & 11.2\% & 3 & em3d & 88.9\% & 88.2\% & 122.5\% & 8,198 & Reductions-dbl & -1.1\% & -1.3\% & -0.6\% & 11 \\
  IRSmk & -0.3\% & -0.4\% & 3.1\% & 29 & health & 12.3\% & 8.2\% & 50.5\% & 1.7M & Reductions-flt & -0.5\% & -0.5\% & 0.8\% & 11 \\
  drop3 & 38.0\% & 19.3\% & 39.5\% & 2 & mst & 99.7\% & 86.2\% & 152.8\% & 797 & Searching-dbl & -0.6\% & -0.3\% & -1.8\% & 11 \\
  five11 & 75.9\% & 70.5\% & 78.3\% & 4,760 & perimeter & 28.4\% & 29.3\% & 67.5\% & 1.4M & Searching-flt & 0.1\% & 0.1\% & -1.9\% & 11 \\
  uudecode & 51.7\% & 49.7\% & 110.0\% & 1 & power & 0.0\% & 0.5\% & 1.5\% & 18k & StatementReordering-dbl & 0.0\% & -0.0\% & 1.4\% & 11 \\
  uuencode & -- & -- & -- & 2 & treeadd & 13.8\% & 13.4\% & 43.4\% & 4.2M & StatementReordering-flt & -0.0\% & 0.8\% & -0.3\% & 11 \\
  bullet & 49.7\% & 40.4\% & 71.3\% & 55k & tsp & 18.7\% & 16.4\% & 21.5\% & 1.0M & Symbolics-dbl & 0.0\% & 0.3\% & 12.4\% & 11 \\
  CLAMR & 32.0\% & 29.7\% & 54.2\% & 220 & voronoi & 81.0\% & 67.5\% & 111.1\% & 2 & Symbolics-flt & 1.9\% & 3.2\% & 8.3\% & 11 \\
  HACCKernels & 4.0\% & 4.5\% & -3.3\% & 7 & paq8p & 45.5\% & 36.9\% & 63.5\% & 324 & enc-3des & 0.9\% & 0.7\% & 0.7\% & 4 \\
  HPCCG & 24.7\% & 23.6\% & 56.8\% & 53 & city & -- & -- & -- & 78 & enc-md5 & 0.3\% & 0.2\% & 0.3\% & 1 \\
  PENNANT & -- & -- & -- & 182k & employ & -- & -- & -- & 2 & enc-pc1 & 9.6\% & 4.7\% & -3.5\% & 3 \\
  miniFE & 74.9\% & 66.2\% & 89.7\% & 25k & life & 91.8\% & 84.8\% & 265.3\% & 4,645 & enc-rc4 & -0.3\% & 0.8\% & -0.1\% & 1 \\
  CoMD & 75.9\% & 58.8\% & 74.7\% & 58 & ocean & 46.8\% & 29.1\% & 32.0\% & 1.0M & netbench-crc & 2.7\% & 1.4\% & 1.1\% & 12k \\
  PathFinder & 83.8\% & 71.5\% & 164.1\% & 17k & primes & 105.7\% & 48.7\% & 53.2\% & 9,593 & netbench-url & -- & -- & -- & 2,803 \\
  rsbench & 18.1\% & 13.2\% & 23.1\% & 38 & simul & -- & -- & -- & 2,003 & 8b10b & 27.8\% & 9.3\% & 50.8\% & 4 \\
  SimpleMOC & 62.9\% & 59.2\% & 66.7\% & 24 & agrep & -- & -- & -- & 2 & beamformer & 31.2\% & 34.6\% & 60.1\% & 2 \\
  XSBench & 66.7\% & 47.5\% & 60.1\% & 32 & mybison & -- & -- & -- & 1,369 & bmm & 0.0\% & 0.2\% & 0.3\% & 3 \\
  miniAMR & 40.9\% & 32.9\% & 55.6\% & 2.2M & gnugo & 110.7\% & 107.8\% & 79.0\% & 2 & dbms & 34.1\% & 25.2\% & 49.4\% & 236k \\
  miniGMG & 61.2\% & 57.0\% & 60.0\% & 214 & anagram & 107.0\% & 94.8\% & 109.1\% & 364 & ecbdes & 5.9\% & 5.4\% & 6.5\% & 6 \\
  fhourstones3.1 & 21.7\% & 13.3\% & 18.5\% & 38 & bc & 71.0\% & 58.5\% & 91.8\% & 2 & llu & 15.5\% & 8.3\% & 20.4\% & 196k \\
  fhourstones & 39.5\% & 30.0\% & 65.3\% & 42 & ft & 50.8\% & 31.1\% & 35.6\% & 2 & pairlocalalign & 38.0\% & 33.6\% & 30.7\% & 2 \\
  analyzer & 130.4\% & 106.0\% & 157.1\% & 16k & ks & 63.8\% & 39.4\% & 115.1\% & 2,019 & rawcaudio & -- & -- & -- & 3 \\
  distray & 35.0\% & 36.4\% & 10.7\% & 2 & yacr2 & 63.1\% & 63.0\% & 108.8\% & 2 & rawdaudio & -- & -- & -- & 2 \\
  fourinarow & 0.5\% & 0.1\% & 0.3\% & 0 & backprop & -15.1\% & -14.6\% & 1.3\% & 11 & encode & 5.0\% & 7.7\% & 12.5\% & 5 \\
  mason & 22.8\% & 25.7\% & 63.2\% & 54 & hotspot & -0.2\% & -0.1\% & 2.3\% & 4 & toast & 19.4\% & 12.0\% & 0.0\% & 28 \\
  neural & 96.6\% & 70.8\% & 44.1\% & 658 & pathfinder & 39.8\% & 30.1\% & 65.4\% & 2 & cjpeg & -- & -- & -- & 18 \\
  pcompress2 & 24.5\% & 20.9\% & 45.3\% & 14 & srad & 4.9\% & 5.8\% & 4.7\% & 8 & mpeg2decode & -- & -- & -- & 45 \\
  pifft & 2.4\% & 2.9\% & 10.4\% & 11 & scimark2 & 30.7\% & 27.6\% & 30.4\% & 205 & nbench & 19.9\% & 23.0\% & 30.1\% & 48 \\
  cfrac & 80.9\% & 68.3\% & 96.5\% & 8,840 & ControlFlow-dbl & 4.6\% & 2.8\% & 9.0\% & 11 & sim & 28.7\% & 22.8\% & 54.7\% & 8,896 \\
  espresso & 58.9\% & 49.9\% & 83.5\% & 4,412 & ControlFlow-flt & 7.2\% & 7.0\% & 14.0\% & 11 & tramp3d-v4 & 47.8\% & 45.8\% & 74.7\% & 1,361 \\
  gs & -- & -- & -- & 6,296 & ControlLoops-dbl & 0.2\% & -0.1\% & 3.0\% & 11 & & & & & \\
  \bottomrule
\end{tabular}


==> eval/tab-llvm-full.tex <==
\begin{table*}[!t]
  \centering
  \caption{Per-program PTSan runtime overhead and peak live object
  IDs on all \LlvmTestCount{} LLVM MultiSource benchmarks (--:
  excluded from overhead measurement, Section~\ref{sec:evaluation:setup}).}
  \label{tab:llvm-full}
  \scriptsize
  \setlength{\tabcolsep}{3pt}
  \resizebox{\textwidth}{!}{\input{eval/generated/tab-llvm-full-body}}
  \Description{Table of per-program PTSan overheads with and without
  LAM, and peak live object-ID counts, for every LLVM MultiSource
  benchmark.}
\end{table*}

